The Empirical Spectral Distribution of i.i.d. Random Matrices with Random Perturbations

A large i.i.d. random matrix with deterministic low-rank perturbation has been extensively studied, particularly in the aspects of the ESD (Empirical Spectral Distribution) and the outliers of eigenvalues. In this work, we investigate the analogous scenario where the perturbation is random and extend the previous results from the deterministic perturbation to the random case. Specifically, we consider an i.i.d. matrix with random perturbation, $\mathbf{M}$. Our results show that: (i) the eigenvalue outliers of $\mathbf{M}$ converge to the eigenvalues of its perturbation; (ii) the ESD of $\mathbf{M}$ converges to the circular law; (iii) the eigenvector alignment holds for specific perturbations. As an application of the above random matrices, we present the first optimal query complexity lower bound for approximating the top eigenvector of asymmetric matrices. In the inverse polynomial accuracy regime, the complexity matches the upper bounds that can be obtained via the power method. As far as we know, it is the first lower bound for approximating the eigenvector of an asymmetric matrix.

==> cover_letter/coverletter.tex <==
% \begin{document}
% \noindent Dear the Editor-in-Chief:

% We would like to submit our manuscript, \textit{``On Non-local Convergence Analysis of Gradient Flow for Deep Linear Networks''} to the Journal of Machine Learning Research (JMLR). All the authors involved with this work have approved the manuscript and agree to its submission.

% In this paper, we study the non-local convergence properties of deep linear networks.
% Specifically, under the quadratic loss, we consider optimizing deep linear networks in which there is at least a layer with only one neuron.
% We describe the convergent point of trajectories with an arbitrary balanced starting point under gradient flow, including the paths which converge to one of the saddle points.
% We also show specific convergence rates of these trajectories by stages with the explicit rates varying from sublinear to linear. 
% As far as we know, our results are the first to give an explicit \textit{non-local} analysis of deep linear neural networks \textit{with arbitrary balanced initialization}, rather than the lazy training regime which has dominated the literature of neural networks.

% \textbf{Notification:} Our submission is an extended version of an earlier conference paper
% (Kun Chen, Dachao Lin, Zhihua Zhang. On Non-local Convergence Analysis of Deep Linear Networks, ICML 2022).
% We have added new contents, including 1) the analysis of the explicit rates of the trajectories that converging to \textit{saddle points} (see our manuscript ``Section 4. Convergence Rates of Trajectories'' for detail), which indeed covers all balanced initialization, while we only show the rates for global minimizers in our conference version. 
% 2) More discussion of $t_2$, such as the concrete examples (Example 4 in Section 4.6), and a theorem avoids this implicit time (Theorem 23), as well as its upper bounds in a limited case (Theorem 25).
% 3) Except the new results, we also have simplified the proofs and fixed some small issues in the original conference version, as well as showing more experiments and examples for improving readability.

% Our suggested action editors are Ohad Shamir, Simon Lacoste-Julien.
% %And our suggested potential reviewers are XXX,XXX,XXX.
% %Quanquan Gu, Tianbao Yang and Lijun Zhang. 
% We have conflicts of interest with Tong Zhang and Zhihua Zhang. 
% Please contact Dachao Lin with any questions about the manuscript.

% We would be grateful if the manuscript could be reviewed and considered for publication in JMLR. 
% If you have any questions, please don't hesitate to contact us. \\

% \noindent Yours sincerely, \\

% \noindent Dachao Lin \\
% lindachao@pku.edu.cn \\
% Academy for Advanced Interdisciplinary Studies \\
% Peking University, Beijing, China \\

% \noindent Kun Chen \\
% kchen0415@pku.edu.cn \\
% School of Mathematical Sciences \\
% Peking University, Beijing, China \\

% \noindent Zhihua Zhang \\
% zhzhang@math.pku.edu.cn \\
% School of Mathematical Sciences \\
% Peking University, Beijing, China
% \end{document}

% !TEX program = pdflatex
\input{coverletter_preamble.tex}
\input{math_commands}

\begin{document}
\hfill{\today}

Advances in Mathematics

\bigskip

Dear the Editor-in-Chief:

We would like to submit our manuscript, \textit{``The Empirical Spectral Distribution of i.i.d.\ Random Matrices with Random Perturbations''} to the Advances in Mathematics. All the authors involved with this work have approved the manuscript and agree to its submission. Here is our abstract:

In this paper, we consider the deformed i.i.d\ matrix $\mM :=\frac{1}{\sqrt{d}}\mW+\mU\mathbf{\Lambda}\mU^*$, where the entries of $\mW$ are i.i.d.\ complex variables with zero mean, unit variance, and finite fourth moment; $\mathbf{\Lambda}=\operatorname{diag}(\lambda_1, \lambda_2, \ldots, \lambda_r)$ is a diagonal matrix with $\lambda_1\ge\lambda_2\ge \ldots\ge \lambda_r>1$ and $\mU$ is uniformly drawn from the Stiefel manifold $\operatorname{Stief}(d,r)$ or its complex counterpart $\operatorname{Stief}_\sC(d,r)$. We consider three aspects of $\mM$:

\begin{itemize}
\item[1.] \textbf{Eigenvalue Outliers and ESD}: We show that the top $r$ eigenvalues of $\mM$ concentrate around $\lambda_1,\lambda_2,\ldots,\lambda_r$, respectively,  and the magnitude of the $(r{+}1)$-th eigenvalue concentrates around $1$, thus extending the previous results from deterministic to random perturbations. Along the proof, we extend the Hanson-Wright inequality to asymmetric and complex settings.

\item[2.] \textbf{Eigenvector Alignment}: For the case $r=1$ (i.e., $\mM=\frac{1}{\sqrt{d}}\mW+\lambda\vu\vu^*$), we prove that the top eigenvector (namely $\vv_1(\mM)$, i.e., the eigenvector corresponding to the top eigenvalue) aligns with $\vu$ in the sense that $\left|\langle\vv_1(\mM), \vu\rangle\right|$ converges to a limit which depends on $\lambda$ (in probability).

\item[3.] \textbf{Eigenvector Approximation}: We present the first optimal \textit{query complexity} lower bound for approximating the top eigenvector of any asymmetric but diagonalizable matrix by analyzing the eigenvector of the random matrix $\mM$ above. More specifically, we show that for every $\operatorname{gap}\in (0,1/2]$ and sufficiently large dimension $d$, there exists a random matrix $\mM$ with $\operatorname{gap}(\mM)=\Omega(\operatorname{gap})$, such that if a matrix-vector product algorithm can identify a vector $\hat\vv$ which satisfies $\left\|\hat{\vv}-\vv_1(\mM) \right\|_2^2\le \operatorname{const}\times \operatorname{gap}$, it needs at least $\mathcal{O}\left(\frac{\log d}{\operatorname{gap}}\right)$ queries of matrix-vector products.

\end{itemize}

% Please contact Kun Chen with any questions about the manuscript.
We would be grateful if the manuscript could be reviewed and considered for publication in Advances in Mathematics. 
If you have any questions, please don't hesitate to contact us. 

\bigskip

Sincerely,

\medskip

Kun Chen \\
kchen0415@pku.edu.cn \\
School of Mathematical Sciences \\
Peking University, Beijing, China \\

Zhihua Zhang \\
zhzhang@math.pku.edu.cn \\
School of Mathematical Sciences \\
Peking University, Beijing, China

\end{document}





